Shaped Gaussian Dictionaries for Quantized Networked Control Systems with Correlated Dropouts

This paper studies fixed rate vector quantisation for noisy networked control systems (NCSs) with correlated packet dropouts. In particular, a discrete-time linear time invariant system is to be controlled over an error-prone digital channel. The controller uses (quantized) packetized predictive control to reduce the impact of packet losses. The proposed vector quantizer is based on sparse regression codes (SPARC), which have recently been shown to be efficient in open-loop systems when coding white Gaussian sources. The dictionaries in existing design of SPARCs consist of independent and identically distributed (i.i.d.) Gaussian entries. However, we show that a significant gain can be achieved by using Gaussian dictionaries that are shaped according to the second-order statistics of the NCS in question. Furthermore, to avoid training of the dictionaries, we provide closed-form expressions for the required second-order statistics in the absence of quantization.

==> Makefile <==
# This makefile ignores files in ./ and in ./cd
# except: .m and .eps files in ./cd
# It must be run twice, to make sure that a complete .m -> .eps -> .pdf has been done
EPSFILES  := $(shell find . -not -path "./cd/*" -path "./*/*.eps")
SVGFILES := $(shell find . -not -path "./cd/*" -path "./*/*.svg")
#PSFILES := $(shell find . -not -path "./cd/*" -path "./*/*.ps")
TIFFFILES := $(shell find . -not -path "./cd/*" -path "./*/*.tiff")

# Filnavne på ønskede pdf filer
EPS_PDFFILES := $(EPSFILES:.eps=.pdf)
#PS_PDFFILES := $(PSFILES:.ps=.pdf)
SVG_PDFFILES := $(SVGFILES:.svg=.pdf)
TIFF_PDFFILES := $(TIFFFILES:.tiff=.pdf)

# PHONY targets
.PHONY: cd
all: figs 
figs: matlab $(PS_PDFFILES) $(SVG_PDFFILES) $(TIFF_PDFFILES) python #pdfcrop $(EPS_PDFFILES)

clean: latexclean
	rm -f $(PS_PDFFILES) $(SVG_PDFFILES) $(TIFF_PDFFILES)  Makefile.md5sums Makefilepy.info 
	touch Makefile.md5sums
	touch Makefilepy.info
	@ echo "***********"
	@ echo "Please note: EPS files created from .m files have NOT been deleted"
	@ echo "***********"

latexclean:
	rm -f main.lox main.fdb_latexmk \
		main.log main.out main.synctex.gz main.toc cdrefs.txt
	rm -f ./*/*.aux ./*/*.bbl ./*/*.blg
	rm -f ./*.aux ./*.bbl ./*.blg

# copies contents of folders in appendix/*/cd to cd/*
cd:	bash -c ' \
		files=$$(find . -wholename "./appendix/*/cd" -type d); \
		for line in $$files; do \
			[[ "$$line" =~ \./appendix/([^/]*)/cd ]]; \
			if [ -e "cd/$${BASH_REMATCH[1]}" ]; then \
				echo "** ERROR: cd/$${BASH_REMATCH[1]} exists."; \
				echo "Use make cdclean to remove"; \
				break; \
			fi; \
			cp -R "appendix/$${BASH_REMATCH[1]}/cd" "cd/$${BASH_REMATCH[1]}"; \
		done'

cdclean:
	bash -c ' \
		files=$$(find . -wholename "./appendix/*/cd" -type d); \
		for line in $$files; do \
			[[ "$$line" =~ \./appendix/([^/]*)/cd ]]; \
			rm -rf "cd/$${BASH_REMATCH[1]}"; \
		done'

cdcheck:
	@ bash -c ' \
		while read line; do \
			file="$$(echo "$$line" | cut -f1 -d" ")"; \
			if [ ! -e "cd/$$file" ]; then \
				echo Not found: "$$file"; \
			fi; \
		done <cdrefs.txt'
	@ echo "Did you remember report?"


# run pdfcrop on all pdffiles that is under svn and has local modifications
# Makefile.md5sums makes sure that pdfcrop is only done once on each file
pdfcrop:
		@- files=$$(hg status | grep "^[AM].*\.pdf$$" | cut -b"9-" | grep -v "^cd/"); \
		for file in $$files; do \
			[ "$$(hg status $$file | grep Untracked)" = "" ] || {\
				echo "******"; \
				echo -e "\tWarning: $$file er ikke under versionsstyring"; \
				echo "******"; }; \
			if [ "$$(grep $$file Makefile.md5sums)" = "$$(md5sum $$file)" ]; then \
				continue; \
			else \
				pdfcrop "$$file" "$$file"; \
				# redirecting directly to grep input file does not work \
				grep --invert-match "$$file" Makefile.md5sums >Makefile.md5sums.new; \
				mv Makefile.md5sums.new Makefile.md5sums; \
				md5sum "$$file" >>Makefile.md5sums; \
			fi \
		done

# .m -> .eps-files
# list of files already converted in Makefile.md5sums
# In the matlab files, create eps-files with:
# print -depsc2 wanted-filename.eps
# These eps files will be converted to pdf
matlab:
		@- files=$$(find .  -not -path "./cd/*" -path "./*/*.m"); \
		for file in $$files; do \
			tempDir=$$PWD; \
			# Look if already run \
			if [ "$$(grep $$file Makefile.info)" = "$$(md5sum $$file)" ]; then \
				continue; \
			fi; \
			# Remove from Makefile.info \
			# redirecting directly to grep input file does not work \
			grep --invert-match "$$file" Makefile.info >Makefile.info.new; \
			mv Makefile.info.new Makefile.info; \
			# Only run files with print lines \
			if [ "$$(grep '^[ 	]*fig2tikz' $$file )" = "" ]; then \
				continue; \
			fi; \
			# Do not execute function scripts \
			if [ "$$(head -n 1 $$file | grep ^function )" != "" ]; then \
				continue; \
			fi; \
			# Run matlab \
			echo -e "******\nRunning matlab on $$file\n******\n"; \
			matlab -nodisplay -r "cd $$(dirname $$file); $$(basename $$file .m);quit"; \
			echo "Changing directory back to $$tempDir";\
			cd $$tempDir;\
			md5sum "$$file" >> Makefile.info; \
		done

python:
		@- files=$$(find .  -not -path "./cd/*" -path "./*/*.py"); \
		for file in $$files; do \
			tempDir=$$PWD; \
			# Look if already run \
			if [ "$$(grep $$file Makefilepy.info)" = "$$(md5sum $$file)" ]; then \
				continue; \
			fi; \
			# Remove from Makefile.info \
			# redirecting directly to grep input file does not work \
			grep --invert-match "$$file" Makefilepy.info >Makefilepy.info.new; \
			mv Makefilepy.info.new Makefilepy.info; \
			# Only run files with savefig lines \
			if [ "$$(grep 'savefig' $$file )" = "" ]; then \
				continue; \
			fi; \
			# Do not execute function scripts \
			if [ "$$(head -n 1 $$file | grep ^function )" != "" ]; then \
				continue; \
			fi; \
			# Run Python \
			echo -e "\n******\nRunning Python on $$file"; \
			echo "Changing directory to $$(dirname $$file)";\
			cd $$(dirname $$file); \
			echo "Running python ..."; \
			output=$$(python2.7 $$(basename $$file)) \
			echo "Changing directory back to $$tempDir"; \
			cd $$tempDir; \
			if [$$output = ""]; then \
				echo "Saving md5sum to Makefilepy.info"; \
				md5sum "$$file" >>Makefilepy.info; \
			else\
				echo "Running python on $$file failed"; \
			fi;\
			echo -e "******"; \
		done


# EPS -> PDF
%.pdf : %.eps
	# @ sed -i -e 's/\\303\\246/\\346/g' -e 's/\\303\\206/\\306/g' \
	# 	 -e 's/\\303\\270/\\370/g' -e 's/\\303\\230/\\330/g' \
	# 	 -e 's/\\303\\245/\\345/g' -e 's/\\303\\205/\\305/g' "$<";
	epstopdf -o "$@" "$<"
	pdfcrop "$@" "$@"
	@# SVN control not done, since most eps files are autogenerated from matlab files

%.pdf : %.ps
	pstopdf -o "$@" "$<"
	pdfcrop "$@" "$@"
	@- [ "$$(hg status $< | grep Untracked)" = "" ] || \
				echo -e "******\n\tWarning: $< is not under versionscontrol\n******"
%.pdf : %.tiff
	tiff2pdf -o "$@" "$<" 
	pdfcrop "$@" "$@"
	@- [ "$$(hg status $< | grep Untracked)" = "" ] || \
				echo -e "******\n\tWarning: $< is not under versionscontrol\n******"	
# SVG -> PDF
%.pdf : %.svg
	inkscape -D -z --file="$<" --export-pdf="$@" --export-latex 
	@- [ "$$(hg status $< | grep Untracked)" = "" ] || \
				echo -e "******\n\tWarning: $< is still not under versioncontrol\n******"

latex:

	pdflatex --shell-escape -file-line-error -halt-on-error mainreport.tex |  sed 's/FiXme Fatal Error//' | sed 's/FiXme Warning//' | grep -e Error -e error
#	texi2pdf main.tex --pdf --quiet --batch
	bibtex mainreport
	pdflatex --shell-escape -halt-on-error mainreport.tex  >> /dev/null 
	pdflatex --shell-escape -file-line-error -halt-on-error mainreport.tex |  sed 's/FiXme Fatal Error//' | sed 's/FiXme Warning//' | grep -e Error -e error -e Warning


==> simulations/fig/mse_rate_singlestate_pd20/single.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{single}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           12-Jan-2014 13:25:59
% eps bounding box:     8.5 cm x 6.697 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s03}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\hspace{0.6cm}{Rate [bit/symbol]}\end{tabular}}%
\psfrag{s04}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\vspace{-0.3cm}{MSE [dB]}\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{3}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{5}%
\psfrag{x04}[t][t]{6}%
%
% yticklabels:
\psfrag{v01}[r][r]{10}%
\psfrag{v02}[r][r]{15}%
\psfrag{v03}[r][r]{20}%
\psfrag{v04}[r][r]{25}%
\psfrag{v05}[r][r]{30}%
%
% Figure:
\resizebox{6.8cm}{!}{\includegraphics{single.eps}}%
\end{psfrags}%
%
% End single.tex


==> simulations/fig/mse_rate_twostate_new/twostate.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{twostate}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           07-Feb-2014 12:59:32
% eps bounding box:     8.5 cm x 6.697 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s03}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\hspace{0.4cm}{Rate [bit/symbol]}\end{tabular}}%
\psfrag{s04}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\vspace{-0.2cm}{MSE [dB]}\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{4.5}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{5.5}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{6.5}%
\psfrag{x06}[t][t]{7}%
%
% yticklabels:
\psfrag{v01}[r][r]{20.5}%
\psfrag{v02}[r][r]{21}%
\psfrag{v03}[r][r]{21.5}%
\psfrag{v04}[r][r]{22}%
\psfrag{v05}[r][r]{22.5}%
\psfrag{v06}[r][r]{23}%
\psfrag{v07}[r][r]{23.5}%
%
% Figure:
\resizebox{6.8cm}{!}{\includegraphics{twostate.eps}}%
\end{psfrags}%
%
% End twostate.tex


==> simulations/fig/mse_rate_twostate_pd25/mjlsgausn.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{mjlsgausn}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           12-Jan-2014 13:25:42
% eps bounding box:     8.5 cm x 6.697 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s03}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\hspace{0.6cm}{Rate [bit/symbol]}\end{tabular}}%
\psfrag{s04}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\vspace{-0.3cm}{MSE [dB]}\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{3}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{5}%
\psfrag{x04}[t][t]{6}%
%
% yticklabels:
\psfrag{v01}[r][r]{10}%
\psfrag{v02}[r][r]{15}%
\psfrag{v03}[r][r]{20}%
\psfrag{v04}[r][r]{25}%
\psfrag{v05}[r][r]{30}%
%
% Figure:
\resizebox{6.8cm}{!}{\includegraphics{mjlsgausn.eps}}%
\end{psfrags}%
%
% End mjlsgausn.tex


==> simulations/fig/mse_rate_twostate_pd25/mjlsgausr.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{mjlsgausr}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           12-Jan-2014 13:25:43
% eps bounding box:     8.5 cm x 7.5192 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s03}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\hspace{0.6cm}{Rate [bit/symbol]}\end{tabular}}%
\psfrag{s04}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\vspace{-0.3cm}{MSE [dB]}\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{3}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{5}%
\psfrag{x04}[t][t]{6}%
%
% yticklabels:
\psfrag{v01}[r][r]{10}%
\psfrag{v02}[r][r]{15}%
\psfrag{v03}[r][r]{20}%
\psfrag{v04}[r][r]{25}%
\psfrag{v05}[r][r]{30}%
%
% Figure:
\resizebox{6.8cm}{!}{\includegraphics{mjlsgausr.eps}}%
\end{psfrags}%
%
% End mjlsgausr.tex


==> simulations/fig/mse_rate_twostate_pd25/mjlslat.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{mjlslat}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           12-Jan-2014 13:25:44
% eps bounding box:     8.5 cm x 7.5192 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s03}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\hspace{0.6cm}{Rate [bit/symbol]}\end{tabular}}%
\psfrag{s04}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\vspace{-0.3cm}{MSE [dB]}\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{3}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{5}%
\psfrag{x04}[t][t]{6}%
%
% yticklabels:
\psfrag{v01}[r][r]{10}%
\psfrag{v02}[r][r]{15}%
\psfrag{v03}[r][r]{20}%
\psfrag{v04}[r][r]{25}%
\psfrag{v05}[r][r]{30}%
%
% Figure:
\resizebox{6.8cm}{!}{\includegraphics{mjlslat.eps}}%
\end{psfrags}%
%
% End mjlslat.tex

